Bootstrapping Fisher Market Equilibrium and First-Price Pacing Equilibrium

The linear Fisher market (LFM) is a basic equilibrium model from economics, which also has applications in fair and efficient resource allocation. First-price pacing equilibrium (FPPE) is a model capturing budget-management mechanisms in first-price auctions. In certain practical settings such as advertising auctions, there is an interest in performing statistical inference over these models. A popular methodology for general statistical inference is the bootstrap procedure. Yet, for LFM and FPPE there is no existing theory for the valid application of bootstrap procedures. In this paper, we introduce and devise several statistically valid bootstrap inference procedures for LFM and FPPE. The most challenging part is to bootstrap general FPPE, which reduces to bootstrapping constrained M-estimators, a largely unexplored problem. We devise a bootstrap procedure for FPPE under mild degeneracy conditions by using the powerful tool of epi-convergence theory. Experiments with synthetic and semi-real data verify our theory.

==> tbl_bsipinyou.tex <==
\begin{table}[ht]
\centering
\caption{Coverage and width of CI in parentheses. $\alpha$ = proportion of $\beta_i = 1$, $d$ is the exponent in bootstrap stepsize $\epsilon_t = t^{-d}$.}
\label{tbl:bsipinyou}
\begin{tabular}{ll|llllllllllllllll}
\toprule
     & $\alpha$ & \multicolumn{4}{l}{0.1} & \multicolumn{4}{l}{0.3} & \multicolumn{4}{l}{0.5} & \multicolumn{4}{l}{0.9} \\
     & buyer &                       10 &                       20 &                       30 &                        50 &                       10 &                       20 &                       30 &                       50 &                       10 &                       20 &                       30 &                       50 &                       10 &                       20 &                       30 &                       50 \\
\midrule $d$ & item &                          &                          &                          &                           &                          &                          &                          &                          &                          &                          &                          &                          &                          &                          &                          &                          \\
\midrule
\multirow{3}{*}{0.40} & 100 &  \makecell{0.55\\(0.70)} &  \makecell{0.75\\(1.27)} &  \makecell{0.58\\(1.93)} &   \makecell{0.61\\(3.45)} &  \makecell{0.73\\(0.80)} &  \makecell{0.76\\(1.32)} &  \makecell{0.49\\(2.22)} &  \makecell{0.18\\(2.94)} &  \makecell{0.81\\(0.75)} &  \makecell{0.84\\(1.45)} &  \makecell{0.77\\(1.83)} &  \makecell{0.14\\(2.25)} &  \makecell{0.66\\(0.79)} &  \makecell{0.58\\(0.99)} &  \makecell{0.35\\(1.17)} &  \makecell{0.47\\(1.61)} \\
     & 300 &  \makecell{0.68\\(0.40)} &  \makecell{0.75\\(0.67)} &  \makecell{0.74\\(0.99)} &    \makecell{0.8\\(1.67)} &  \makecell{0.82\\(0.49)} &  \makecell{0.82\\(0.72)} &  \makecell{0.83\\(1.32)} &  \makecell{0.46\\(1.83)} &  \makecell{0.82\\(0.44)} &   \makecell{0.8\\(0.86)} &   \makecell{0.9\\(1.19)} &  \makecell{0.32\\(1.60)} &  \makecell{0.83\\(0.49)} &  \makecell{0.73\\(0.61)} &  \makecell{0.67\\(0.78)} &  \makecell{0.73\\(0.98)} \\
     & 500 &  \makecell{0.75\\(0.30)} &  \makecell{0.66\\(0.51)} &  \makecell{0.78\\(0.75)} &   \makecell{0.81\\(1.20)} &  \makecell{0.87\\(0.38)} &  \makecell{0.89\\(0.54)} &   \makecell{0.8\\(1.04)} &  \makecell{0.81\\(1.46)} &  \makecell{0.91\\(0.33)} &  \makecell{0.89\\(0.69)} &  \makecell{0.82\\(0.95)} &  \makecell{0.51\\(1.37)} &  \makecell{0.87\\(0.37)} &  \makecell{0.76\\(0.47)} &  \makecell{0.77\\(0.60)} &  \makecell{0.84\\(0.76)} \\
\cline{1-18}
\multirow{3}{*}{0.30} & 100 &   \makecell{0.8\\(1.07)} &  \makecell{0.92\\(2.05)} &  \makecell{0.83\\(2.90)} &   \makecell{0.92\\(5.19)} &  \makecell{0.92\\(1.20)} &  \makecell{0.88\\(1.99)} &  \makecell{0.82\\(3.30)} &  \makecell{0.24\\(4.07)} &  \makecell{0.88\\(1.16)} &  \makecell{0.93\\(2.06)} &   \makecell{0.9\\(2.52)} &  \makecell{0.38\\(3.19)} &  \makecell{0.82\\(1.07)} &  \makecell{0.78\\(1.43)} &  \makecell{0.65\\(1.71)} &   \makecell{0.7\\(2.26)} \\
     & 300 &  \makecell{0.87\\(0.71)} &  \makecell{0.96\\(1.19)} &  \makecell{0.89\\(1.73)} &   \makecell{0.94\\(2.80)} &  \makecell{0.94\\(0.83)} &  \makecell{0.93\\(1.22)} &  \makecell{0.94\\(2.19)} &  \makecell{0.73\\(2.93)} &  \makecell{0.93\\(0.76)} &  \makecell{0.97\\(1.44)} &  \makecell{0.96\\(1.93)} &  \makecell{0.41\\(2.53)} &   \makecell{0.9\\(0.76)} &   \makecell{0.9\\(0.99)} &  \makecell{0.87\\(1.23)} &  \makecell{0.87\\(1.59)} \\
     & 500 &  \makecell{0.85\\(0.56)} &  \makecell{0.92\\(0.94)} &   \makecell{0.9\\(1.34)} &   \makecell{0.94\\(2.16)} &  \makecell{0.95\\(0.68)} &  \makecell{0.97\\(0.97)} &  \makecell{0.95\\(1.85)} &  \makecell{0.91\\(2.59)} &   \makecell{0.9\\(0.60)} &  \makecell{0.97\\(1.20)} &  \makecell{0.99\\(1.63)} &  \makecell{0.82\\(2.16)} &  \makecell{0.98\\(0.62)} &  \makecell{0.96\\(0.79)} &  \makecell{0.94\\(1.01)} &  \makecell{0.96\\(1.27)} \\
\cline{1-18}
\multirow{3}{*}{0.20} & 100 &  \makecell{0.95\\(1.59)} &  \makecell{0.93\\(2.93)} &  \makecell{0.95\\(4.11)} &   \makecell{0.97\\(7.22)} &  \makecell{0.95\\(1.73)} &   \makecell{1.0\\(2.91)} &  \makecell{0.85\\(4.32)} &  \makecell{0.56\\(5.43)} &  \makecell{0.95\\(1.65)} &  \makecell{0.99\\(2.87)} &  \makecell{0.94\\(3.34)} &  \makecell{0.38\\(4.15)} &  \makecell{0.84\\(1.46)} &  \makecell{0.91\\(1.94)} &  \makecell{0.78\\(2.26)} &  \makecell{0.85\\(3.01)} \\
     & 300 &  \makecell{0.98\\(1.17)} &  \makecell{0.98\\(1.97)} &  \makecell{0.98\\(2.78)} &   \makecell{0.99\\(4.52)} &  \makecell{0.98\\(1.34)} &   \makecell{1.0\\(1.93)} &  \makecell{0.99\\(3.22)} &  \makecell{0.79\\(4.42)} &  \makecell{0.99\\(1.19)} &  \makecell{0.98\\(2.16)} &   \makecell{1.0\\(2.76)} &  \makecell{0.84\\(3.54)} &  \makecell{0.98\\(1.11)} &  \makecell{0.99\\(1.55)} &  \makecell{0.95\\(1.80)} &  \makecell{0.96\\(2.29)} \\
     & 500 &   \makecell{1.0\\(1.01)} &   \makecell{1.0\\(1.66)} &   \makecell{1.0\\(2.37)} &    \makecell{1.0\\(3.69)} &  \makecell{0.99\\(1.14)} &   \makecell{1.0\\(1.68)} &   \makecell{1.0\\(2.87)} &   \makecell{1.0\\(3.84)} &   \makecell{1.0\\(1.04)} &   \makecell{1.0\\(1.96)} &   \makecell{1.0\\(2.47)} &  \makecell{0.93\\(3.30)} &   \makecell{1.0\\(1.00)} &  \makecell{0.99\\(1.33)} &  \makecell{0.99\\(1.60)} &  \makecell{0.99\\(2.02)} \\
\cline{1-18}
\multirow{3}{*}{0.10} & 100 &  \makecell{0.98\\(2.18)} &  \makecell{0.99\\(3.96)} &  \makecell{0.99\\(5.58)} &    \makecell{1.0\\(9.56)} &   \makecell{1.0\\(2.21)} &  \makecell{0.99\\(3.96)} &  \makecell{0.95\\(5.30)} &  \makecell{0.62\\(6.73)} &  \makecell{0.98\\(2.10)} &  \makecell{0.99\\(3.47)} &  \makecell{0.99\\(4.13)} &  \makecell{0.52\\(4.94)} &  \makecell{0.96\\(1.74)} &   \makecell{0.9\\(2.38)} &  \makecell{0.92\\(2.73)} &  \makecell{0.94\\(3.67)} \\
     & 300 &   \makecell{1.0\\(1.76)} &   \makecell{1.0\\(2.96)} &   \makecell{1.0\\(4.12)} &    \makecell{1.0\\(6.48)} &  \makecell{0.99\\(1.88)} &   \makecell{1.0\\(2.89)} &   \makecell{1.0\\(4.24)} &  \makecell{0.97\\(5.53)} &   \makecell{1.0\\(1.79)} &   \makecell{1.0\\(2.78)} &   \makecell{1.0\\(3.56)} &  \makecell{0.98\\(4.42)} &   \makecell{1.0\\(1.53)} &   \makecell{1.0\\(2.05)} &   \makecell{1.0\\(2.30)} &   \makecell{1.0\\(2.98)} \\
     & 500 &   \makecell{1.0\\(1.59)} &   \makecell{1.0\\(2.60)} &   \makecell{1.0\\(3.61)} &    \makecell{1.0\\(5.42)} &   \makecell{1.0\\(1.74)} &   \makecell{1.0\\(2.64)} &   \makecell{1.0\\(3.84)} &   \makecell{1.0\\(5.06)} &   \makecell{1.0\\(1.62)} &   \makecell{1.0\\(2.71)} &   \makecell{1.0\\(3.38)} &  \makecell{0.99\\(4.28)} &   \makecell{1.0\\(1.37)} &   \makecell{1.0\\(1.80)} &   \makecell{1.0\\(2.19)} &   \makecell{1.0\\(2.69)} \\
\cline{1-18}
\multirow{3}{*}{0.05} & 100 &  \makecell{0.98\\(2.45)} &   \makecell{1.0\\(4.51)} &   \makecell{1.0\\(6.36)} &  \makecell{0.99\\(10.40)} &   \makecell{1.0\\(2.56)} &  \makecell{0.99\\(4.45)} &  \makecell{0.99\\(5.69)} &  \makecell{0.73\\(7.06)} &  \makecell{0.99\\(2.38)} &   \makecell{1.0\\(3.74)} &  \makecell{0.97\\(4.27)} &  \makecell{0.62\\(5.42)} &  \makecell{0.95\\(1.86)} &  \makecell{0.93\\(2.56)} &  \makecell{0.95\\(2.92)} &  \makecell{0.97\\(4.01)} \\
     & 300 &   \makecell{1.0\\(2.05)} &   \makecell{1.0\\(3.39)} &   \makecell{1.0\\(4.65)} &    \makecell{1.0\\(7.26)} &   \makecell{1.0\\(2.15)} &   \makecell{1.0\\(3.30)} &   \makecell{1.0\\(4.61)} &  \makecell{0.99\\(6.02)} &   \makecell{1.0\\(2.02)} &   \makecell{1.0\\(3.20)} &   \makecell{1.0\\(3.90)} &  \makecell{0.97\\(4.87)} &  \makecell{0.98\\(1.63)} &   \makecell{1.0\\(2.28)} &  \makecell{0.99\\(2.57)} &   \makecell{1.0\\(3.23)} \\
     & 500 &   \makecell{1.0\\(1.90)} &   \makecell{1.0\\(3.07)} &   \makecell{1.0\\(4.13)} &    \makecell{1.0\\(6.26)} &   \makecell{1.0\\(2.02)} &   \makecell{1.0\\(2.99)} &   \makecell{1.0\\(4.30)} &   \makecell{1.0\\(5.59)} &   \makecell{1.0\\(1.86)} &   \makecell{1.0\\(2.94)} &   \makecell{1.0\\(3.71)} &   \makecell{1.0\\(4.55)} &   \makecell{1.0\\(1.42)} &   \makecell{1.0\\(2.05)} &   \makecell{1.0\\(2.34)} &   \makecell{1.0\\(2.97)} \\
\bottomrule
\end{tabular}
\end{table}


==> tbl_ipinyou.tex <==
\begin{table}
\centering
\caption{Average CTR (0.01\%) in the week of 2013/06/06--2013/06/12.}
\label{tbl:ctrbyregion}
\begin{tabular}{lrrrrr}
\toprule
Advertizer &  Ecommerce &  Software &  International Ecom &   Oil &  Tire \\
Region         &            &           &                     &       &       \\
\midrule
unknown        &      10.55 &     23.24 &               15.49 & 13.71 &  5.86 \\
Beijing        &       8.37 &      8.38 &                8.36 &  8.14 &  5.20 \\
Tianjin        &       8.22 &     11.40 &                8.56 &  9.53 &  7.06 \\
Hebei          &      11.10 &      7.37 &                8.52 &  8.71 &  8.79 \\
Shanxi         &       9.86 &      8.83 &               10.66 & 10.82 &  6.61 \\
Inner Mongolia &       7.63 &     14.47 &                9.37 &  8.72 &  5.90 \\
Liaoning       &       7.92 &      7.85 &                8.20 &  8.24 &  4.98 \\
Jilin          &       8.74 &      4.56 &                6.83 & 12.04 &  8.14 \\
Heilongjiang   &       9.63 &      5.50 &                8.91 &  7.06 &  4.09 \\
Shanghai       &      10.27 &      7.30 &                9.62 &  6.15 &  3.94 \\
Jiangsu        &       8.13 &      8.55 &                8.99 &  7.36 &  4.10 \\
Zhejiang       &       7.73 &      7.77 &                8.11 & 10.13 &  5.75 \\
Anhui          &      10.36 &      8.77 &                6.58 & 10.23 &  6.03 \\
Fujian         &       6.65 &      8.86 &                9.31 &  7.04 &  5.27 \\
Jiangxi        &      10.32 &      9.40 &                8.68 & 12.00 &  4.70 \\
Shandong       &       8.53 &     10.76 &                7.93 &  9.08 &  5.58 \\
Henan          &       9.10 &      7.15 &                7.66 &  8.15 &  5.73 \\
Hubei          &       6.58 &      7.78 &               11.37 &  7.35 &  5.45 \\
Hunan          &       8.36 &      6.23 &                9.92 &  9.98 &  5.00 \\
Guangdong      &       7.20 &      7.06 &                8.16 &  7.50 &  5.08 \\
Guangxi        &       6.96 &      8.12 &                7.77 &  7.57 &  4.98 \\
Hainan         &       6.99 &     21.07 &               15.48 & 13.72 &  3.29 \\
Chongqing      &       8.64 &      6.14 &                5.43 &  4.61 &  3.44 \\
Sichuan        &       8.19 &      8.33 &                6.07 &  5.59 &  5.28 \\
Guizhou        &      11.49 &     11.51 &               12.93 &  6.20 &  4.76 \\
Yunnan         &      10.02 &      8.50 &                7.73 &  7.15 &  6.53 \\
Xizang         &       9.52 &     29.15 &                9.16 & 31.53 & 10.43 \\
Shannxi        &       8.14 &      7.58 &                8.63 &  8.23 &  7.94 \\
Gansu          &       9.06 &     12.80 &                6.40 & 10.47 &  6.48 \\
Qinghai        &      14.18 &     14.98 &               14.62 &  7.39 &  7.33 \\
Ningxia        &      11.07 &      2.44 &                6.99 & 10.73 &  8.15 \\
Xinjiang       &       6.45 &     10.60 &                7.25 &  7.08 &  4.26 \\
Taiwan         &      10.89 &     17.82 &               24.07 &  8.38 &  1.61 \\
Hong Kong      &       6.39 &     18.90 &               19.36 &  8.87 &  2.31 \\
Macao          &       0.00 &    175.02 &               19.84 & 45.71 &  0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tbl_rev_coverage.tex <==
\begin{tabular}{lllllllllll}
\toprule
 & number of buyers & \multicolumn{3}{r}{20} & \multicolumn{3}{r}{50} & \multicolumn{3}{r}{80} \\
 & beta = 1 proportion & 0.00 & 0.10 & 0.20 & 0.00 & 0.10 & 0.20 & 0.00 & 0.10 & 0.20 \\
d & number of items &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{2}{*}{0.40} & 400 & (1.0, 0.27034895029039335, 1.0, 0.30179918215507473) & (0.85, 0.3291461489113756, 0.87, 0.3276181046287483) & (0.92, 0.47021425883191126, 0.9, 0.4645006631074529) & (1.0, 0.33863902379751826, 1.0, 0.3564745304137062) & (0.91, 0.5008529861522326, 0.86, 0.4984743598145567) & (0.93, 0.5188844255141831, 0.88, 0.5174071411073161) & (1.0, 0.29592282329307557, 1.0, 0.30525033773362004) & (0.9, 0.5108146266267123, 0.92, 0.515807260561256) & (0.88, 0.5469271876521838, 0.91, 0.541726793746458) \\
 & 600 & (1.0, 0.22345337424950173, 1.0, 0.24788735890843988) & (0.86, 0.27161668763190955, 0.84, 0.26713687581369255) & (0.91, 0.38251044071819024, 0.87, 0.3856080296914473) & (1.0, 0.27855091445894054, 1.0, 0.29220346682319004) & (0.83, 0.40807444717197, 0.87, 0.408080167319336) & (0.9, 0.4214881182939701, 0.92, 0.4263303405366047) & (1.0, 0.24121796283164684, 1.0, 0.2509807818648618) & (0.91, 0.422816436131096, 0.86, 0.42094111113401544) & (0.8, 0.4439197161595521, 0.95, 0.4429381379239249) \\
\cline{1-11}
\multirow[t]{2}{*}{0.333333} & 400 & (1.0, 0.27124932193594853, 1.0, 0.301589446874207) & (0.83, 0.3210980832512114, 0.86, 0.3258823015120573) & (0.84, 0.4675646033626249, 0.87, 0.4663867732075794) & (1.0, 0.33717006840751623, 1.0, 0.3563817315455375) & (0.93, 0.49605741690421795, 0.92, 0.49334186324774776) & (0.91, 0.515270015617082, 0.89, 0.520587814278868) & (1.0, 0.2924382583481885, 1.0, 0.30640694999496776) & (0.89, 0.5118900352043098, 0.9, 0.5104533916868964) & (0.89, 0.5475536836594153, 0.9, 0.5392267161777664) \\
 & 600 & (1.0, 0.2230708292176148, 1.0, 0.24752781102185142) & (0.81, 0.26766252444427396, 0.76, 0.2659766580515851) & (0.83, 0.38304593320206637, 0.92, 0.3816661413930484) & (1.0, 0.2792617025602137, 1.0, 0.29240704623008956) & (0.9, 0.4075155827834454, 0.86, 0.4043979410761127) & (0.89, 0.42484039419156766, 0.88, 0.4188703090398753) & (1.0, 0.24023803965396262, 1.0, 0.25081832399579695) & (0.87, 0.4230384188509679, 0.85, 0.41793611612737047) & (0.94, 0.4441146262945933, 0.92, 0.4451014339516163) \\
\cline{1-11}
\multirow[t]{2}{*}{0.166667} & 400 & (1.0, 0.2718675500644464, 1.0, 0.3029625622049007) & (0.82, 0.32871760174969694, 0.85, 0.32551690192651017) & (0.9, 0.4744077725476009, 0.94, 0.4664239809687725) & (1.0, 0.33994456946729884, 1.0, 0.3580169141165658) & (0.95, 0.4994295871510971, 0.89, 0.4978394670916258) & (0.92, 0.5203814561123141, 0.95, 0.5148377943583634) & (1.0, 0.29613776393147756, 1.0, 0.30325356433338335) & (0.9, 0.5198420689646851, 0.87, 0.5185307529745156) & (0.87, 0.5429357816667156, 0.89, 0.5400863287763109) \\
 & 600 & (1.0, 0.22284897847691684, 1.0, 0.24833686725511178) & (0.89, 0.2690642418580509, 0.9, 0.2658474016121947) & (0.84, 0.3872832429116231, 0.89, 0.38087408278781965) & (1.0, 0.27731896449911864, 1.0, 0.29284753289592375) & (0.85, 0.40788357084573007, 0.91, 0.4080512239985652) & (0.81, 0.41913891757817895, 0.92, 0.4220554047587063) & (1.0, 0.24178591245901174, 1.0, 0.25171864490769025) & (0.88, 0.422640743571097, 0.95, 0.4224632294305623) & (0.92, 0.4450669177262664, 0.91, 0.447943056024513) \\
\cline{1-11}
\multirow[t]{2}{*}{0.083333} & 400 & (1.0, 0.2719791235559764, 1.0, 0.3027960025825653) & (0.88, 0.3272949077775246, 0.9, 0.3276016596305487) & (0.91, 0.46802207326569223, 0.89, 0.46619074738660743) & (1.0, 0.33634285567646827, 1.0, 0.3559958761675092) & (0.93, 0.5039960121122462, 0.86, 0.4964403019540491) & (0.81, 0.5229173664899293, 0.83, 0.5134715117739701) & (1.0, 0.29498778803365333, 1.0, 0.3050617457290866) & (0.87, 0.5150696103987413, 0.91, 0.5140715514653857) & (0.9, 0.5426406679195648, 0.88, 0.5408337665718226) \\
 & 600 & (1.0, 0.2241053790808007, 1.0, 0.24669730356642589) & (0.91, 0.26880823530525105, 0.85, 0.2665869826624104) & (0.94, 0.3830899452898398, 0.92, 0.38086204331618456) & (1.0, 0.28013218814855034, 1.0, 0.2911969701325777) & (0.91, 0.4071943975506921, 0.84, 0.40099240756870635) & (0.89, 0.4234217554062236, 0.94, 0.422038115749465) & (1.0, 0.24156952502096857, 1.0, 0.25136473519763236) & (0.91, 0.42121226161152714, 0.93, 0.42331118325582245) & (0.96, 0.4443593683534563, 0.96, 0.44346401670687136) \\
\cline{1-11}
\multirow[t]{2}{*}{0.066667} & 400 & (1.0, 0.27221460536520053, 1.0, 0.3014028346638398) & (0.84, 0.3284056445886342, 0.87, 0.32543143216310233) & (0.92, 0.4711159103271194, 0.95, 0.4638358689514219) & (1.0, 0.3383032097391585, 1.0, 0.3572526828154556) & (0.88, 0.49336730928066735, 0.86, 0.49645942923196434) & (0.9, 0.5126348629083121, 0.86, 0.5143912659270832) & (1.0, 0.2944487568361594, 1.0, 0.30770431631531714) & (0.92, 0.5096862343525064, 0.93, 0.511953344855862) & (0.89, 0.5436572316374811, 0.95, 0.5428669432104936) \\
 & 600 & (1.0, 0.22335179555616066, 1.0, 0.24545444392580215) & (0.81, 0.2687461368299956, 0.91, 0.2692605762659796) & (0.92, 0.38277735204194796, 0.96, 0.37777685806028855) & (1.0, 0.27830859450469814, 1.0, 0.29235600641715176) & (0.9, 0.40657718348237415, 0.88, 0.40563066189649666) & (0.93, 0.4231765531866661, 0.91, 0.4227224251764072) & (1.0, 0.24112401495334243, 1.0, 0.25126400858546033) & (0.88, 0.42052170841006464, 0.86, 0.4215675572408902) & (0.89, 0.44644168033864384, 0.85, 0.44540069214213923) \\
\cline{1-11}
\bottomrule
\end{tabular}

